Kaluza-Klein theory for type $II \ b$ supergravity on the warped deformed conifold

We discuss Kaluza-Klein theory for type $II\ b $ supergravity on the warped deformed conifold using a large radial distance limit of Klebanov-Strassler solution where the radial coordinate separates from angle coordinates for a background asymptotic to $ AdS _5 \times T^{1,1}$ spacetime. The decomposition of field fluctuations on harmonics of the base manifold $T^{1,1}$ and plane waves of $M_4= \dh (AdS _5 )$ is examined for the metric tensor components along $M_4= \dh (AdS _5 )$, the axio-dilaton and the 4-form potential components along $T^{1,1}$. Semi-classical methods are used to compute the mass spectra, wave functions and interactions for a set of modes in low dimensional representations of the isometry group. Deformations of the background solution due to compactification effects are also considered. The information on warped modes properties is utilized to explore the thermal evolution of a cosmic component of metastable modes after exit from brane inflation.

==> revstyle.tex <==
% fichier revstyle.tex 
\hfuzz =1pt
\overfullrule =0pt
\newcounter{subequation}[equation]
\makeatletter \fussy \flushbottom
\def \GUT { grand unified theories }
\def \wrt { with respect to }
\def \cft { conformal field theory }
\def \dof { degrees of freedom }
\def \bef { $\beta -$function }
\def \bet { beta function }
\def \mow { modular weights }
\def \loe { low energy }
\def \km { Kac-Moody }
\def \susy { supersymmetry }
\def \susyq { supersymmetric }
\def \sig { $\sigma -$model }
\def \ws { world sheet }
\def \tres { threshold corrections }
\def \L {\Lambda }
\def \l {\lambda } 
\def \ka {\kappa } 
\def \t {\theta }
\def \vt {\vartheta }
\def \T {\Theta }
\def \vT {\hat {\vartheta } }
\def \a {\alpha }
\def \dh {\partial }
\def \d {\delta }
\def \D {\Delta }
\def \bq {\bar q }
\def \bQ {\bar Q}
\def \g {\gamma }
\def \G {\Gamma }
\def \O {\Omega }
\def \o {\omega }
\def \b {\beta }
\def \S {\Sigma }
\def \s {\sigma }
\def \e {\epsilon }
\def \cc { coupling constant }
\def \ccs {coupling constants }
\def \ph { phenomenology } 
\def \pheny { phenomenologically } 
\def \rhs { right hand side } 
\def \lhs {left  hand side } 
\def \ren { renormalization } 
\def \rge { renormalization group equations}
\def \ud { {1 \over 2} } 
\def \ut { {1 \over 3} } 
\def \td {{3 \over  2 }} 
\def \sm { standard model }
\def \q {\eqno  }
\def \mssm { minimal supersymmetric standard model } 
\def \he  { high energy }
\def \st { string theory }
\def \ft { field theory }
\def \cddd { {\cal D } }
\def \cala { {\cal A } }
\def \calc { {\cal C } }
\def \calp { {\cal P } }
\def \caly { {\cal Y } }
\def \calf { {\cal F } }
\def \calg { {\cal G } }
\def \calq { {\cal Q } }
\def \caln { {\cal N } }
\def \call { {\cal L } }
\def \cale { {\cal E } }
\def \calG { {\cal G } }
\def \calH { {\cal H } }
\def \calk { {\cal K } }
\def \calt { {\Theta } }
\def \calT { {\cal T } }
\def \cald { {\cal D } }
\def \cali { {\cal I } }
\def \calj { {\cal J } }
\def \calb { {\cal B } }
\def \calm { {\cal M } }
\def \calr { {\cal R } }
\def \cals { {\cal S } }
\def \calu { {\cal U } }
\def \calo { {\cal O } }
\def \calz { {\cal z } }
\def \cals { {\cal S } }
\def \calv { {\cal V } }
\def \calx { {\cal X } }
\def \calY { {\cal Y } }
\def \ua  {\underline {a}}
\def \ub  {\underline {b}}
\def \uc  {\underline {c}}
\def \ul  {\underline {l}}
\def \um  {\underline {m}}
\def \un  {\underline {n}}
\def \uA  {\underline {A}}
\def \uB  {\underline {B}}
\def \umg  {\underline {\mu }}
\def \ung  {\underline {\nu }}
\def \ui  {\underline { i }}
\def \uj  {\underline {j}}
\def \uag  {\underline {\alpha }}
\def \ubg  {\underline {\beta }}
\def  \bR  {\textbf  {R}}
\def  \bC   {\textbf{C}}
%\def \bea {\begin{equation}}
%\def \eea {\end{equation}}
\def \tchi  {{\tilde \chi }}
\def \Eslash {E \kern-.5em\slash}
\def \epslash {\epsilon \kern-.5em\slash}
\def \pslash {p \kern-.5em\slash}
\def \kslash {k \kern-.5em\slash}
\def \Dslash {D \kern-.5em\slash}
\def \hslash {h \kern-.5em\slash}
\def \dslash {\partial \kern-.5em\slash}
\def \vslash {v \kern-.5em\slash}
\def \Gslash {G \kern-.5em\slash}
\def \Hslash {H \kern-.5em\slash}
\def \Fslash {F \kern-.5em\slash}
\def \oslash {o \kern-.5em\slash}
\def \bull {$\bullet  \quad $}
\def \bfA { {\bf A} }
\def \bfB { {\bf B} }
\def \bfS { {\bf S} }
\def \jmp { Jour. Math. Phys. }
\def \ptp { Prog. Theor. Phys. }
\def \ap {Ann. Phys. (NY) }
\def \z {Z. Phys. } 
\def \pr  { Phys. Rev. }
\def \np { Nucl. Phys. }  
\def \arr { Ann. Rev. Nucl. Sci. } 
\def \ar { Ann. Rev. Nucl. Part. Sci. } 
\def \pp { Phys. Reports } 
\def \je { Sov. Phys. JETP } 
\def \prl { Phys. Rev. Lett. } 
\def \pl { Phys. Lett. }
\def \rmp { Rev. Mod. Phys. } 
\def \nc { Nuovo Cimento }
\def \jnp { Sov. Jour. Nucl. Phys. }
\def\NPB#1#2#3 {{\rm Nucl.~Phys.}  {\bf{B#1}}, {#3} (#2)}
\def\NPA#1#2#3 {{\rm Nucl.~Phys.}  {\bf{A#1}}, {#3} (#2)}
\def\PLB#1#2#3 {{\rm Phys.~Lett.}  {\bf{B#1}}, {#3} (#2)}
\def\PR#1#2#3 {{\rm Phys.~Rep.}  {\bf#1}, {#3} (#2)} 
\def\PRD#1#2#3 {{\rm Phys.~Rev.}  {\bf{D#1}}, {#3} (#2)} 
\def\PRL#1#2#3  {{\rm Phys.~Rev.~Lett.}  {\bf{#1}}, {#3} (#2)} 
\def\ZPC#1#2#3 {{\rm Z.~Phys.}  {\bf C#1}, {#3} (#2)} 
\def\JHEP#1#2#3 {{\rm JHEP} {\bf C#1}, {#3}  (#2)}     
\def\IJMP#1#2#3 {{\rm Int. J. Mod. Phys.}  {\bf A#1}, {#3} (#2)} 
\def\JMP#1#2#3 {{\rm J. Math. Phys.}  {\bf #1}, {#3} (#2)}
\def\PTP#1#2#3 {{\rm Prog. Theor. Phys.}  {\bf{#1}}, {#3} (#2)}
\def\FP#1#2#3  {{\rm  Fortsch. Phys.}  {\bf{#1}}, {#3} (#2)}
\def\CMP#1#2#3  {{\rm Comm. Math. Phys.}  {\bf{#1}}, {#3} (#2)}
\def\RMP#1#2#3  {{\rm Rev.  Mod. Phys.}  {\bf{#1}}, {#3} (#2)}
%%%%%%RICCI PACKAGE %%%%%%%%%%%%%
\def\mysavedown#1{\edef\mysubs{\mysubs#1}}
\def\mysaveup#1{\edef\mysups{\mysups#1}}
\def\mydown#1{{\mytensor}_{\vphantom{\mysubs}#1}}
\def\myup#1{{\mytensor}^{\vphantom{\mysups}#1}}
\def\tensor#1#2{
  #1
  \def\mytensor{\vphantom{#1}}
  \def\mysubs{\relax}
  \def\mysups{\relax}
% Make one pass across indices to determine maximum height.
  \let\down=\mysavedown
  \let\up=\mysaveup
  #2
% Now make a second pass to typeset the sub- & superscripts.
  \let\down=\mydown
  \let\up=\myup
  #2
  }
\def\Alt{\mathop{\hbox{Alt}}\nolimits}
\def\Sym{\mathop{\hbox{Sym}}\nolimits}
\def\Del{\mathop\nabla\nolimits}
\def\grad{\mathop{\hbox{grad}}\nolimits}
\def\div{\mathop{\hbox{div}}\nolimits}
\def\extd{\mathop{d}\nolimits}
\def\Lie{\cal L} 
%% Change this to "\Cal L" for amstex

%\rightline {hep-th/}
%\rightline  {T98/}
%\hoffset-1in
%\voffset-1in
%\if@twoside\oddsidemargin15mm
%\evensidemargin15mm\marginparwidth15mm
%\else\oddsidemargin15mm\evensidemargin15mm\marginparwidth15mm\fi
%\footheight12pt\footskip30pt
%\textwidth 18 cm
%\baselineskip15pt
%\textheight 45\baselineskip
%\makeatletter
%Subequations
\def\thesubequation{\theequation\@alph\c@subequation}
\def\@subeqnnum{{\rm (\thesubequation)}}
\def\slabel#1{\@bsphack\if@filesw {\let\thepage\relax
   \xdef\@gtempa{\write\@auxout{\string
      \newlabel{#1}{{\thesubequation}{\thepage}}}}}\@gtempa
   \if@nobreak \ifvmode\nobreak\fi\fi\fi\@esphack}
\def\subeqnarray{\stepcounter{equation}
\let\@currentlabel=\theequation\global\c@subequation\@ne
\global\@eqnswtrue
\global\@eqcnt\z@\tabskip\@centering\let\\=\@subeqncr
$$\halign to \displaywidth\bgroup\@eqnsel\hskip\@centering
  $\displaystyle\tabskip\z@{##}$&\global\@eqcnt\@ne
  \hskip 2\arraycolsep \hfil${##}$\hfil
  &\global\@eqcnt\tw@ \hskip 2\arraycolsep
  $\displaystyle\tabskip\z@{##}$\hfil
   \tabskip\@centering&\llap{##}\tabskip\z@\cr}
\def\endsubeqnarray{\@@subeqncr\egroup
                     $$\global\@ignoretrue}
\def\@subeqncr{{\ifnum0=`}\fi\@ifstar{\global\@eqpen\@M
    \@ysubeqncr}{\global\@eqpen\interdisplaylinepenalty \@ysubeqncr}}
\def\@ysubeqncr{\@ifnextchar [{\@xsubeqncr}{\@xsubeqncr[\z@]}}
\def\@xsubeqncr[#1]{\ifnum0=`{\fi}\@@subeqncr
   \noalign{\penalty\@eqpen\vskip\jot\vskip #1\relax}}
\def\@@subeqncr{\let\@tempa\relax
    \ifcase\@eqcnt \def\@tempa{& & &}\or \def\@tempa{& &}
      \else \def\@tempa{&}\fi
     \@tempa \if@eqnsw\@subeqnnum\refstepcounter{subequation}\fi
     \global\@eqnswtrue\global\@eqcnt\z@\cr}
\let\@ssubeqncr=\@subeqncr
\@namedef{subeqnarray*}{\def\@subeqncr{\nonumber\@ssubeqncr}\subeqnarray}
\@namedef{endsubeqnarray*}{\global\advance\c@equation\m@ne%
                           \nonumber\endsubeqnarray}


%Number equations by section
\@addtoreset{equation}{section}
\renewcommand{\theequation}{\thesection.\arabic{equation}}
%Other macros
%\newcommand{\bm}{\bibitem}
\newcommand{\be}{\begin{equation}} 
\newcommand{\ee}{\end{equation}} 
\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\bea}{\begin{eqnarray}} 
\newcommand{\eea}{\end{eqnarray}} 
\newcommand{\bsea}{\begin{subeqnarray}} 
\newcommand{\esea}{\end{subeqnarray}}
\newcommand{\nn}{\nonumber}






